Referencing Where to Focus: Improving VisualGrounding with Referential Query

Visual Grounding aims to localize the referring object in an image given a natural language expression. Recent advancements in DETR-based visual grounding methods have attracted considerable attention, as they directly predict the coordinates of the target object without relying on additional efforts, such as pre-generated proposal candidates or pre-defined anchor boxes. However, existing research primarily focuses on designing stronger multi-modal decoder, which typically generates learnable queries by random initialization or by using linguistic embeddings. This vanilla query generation approach inevitably increases the learning difficulty for the model, as it does not involve any target-related information at the beginning of decoding. Furthermore, they only use the deepest image feature during the query learning process, overlooking the importance of features from other levels. To address these issues, we propose a novel approach, called RefFormer. It consists of the query adaption module that can be seamlessly integrated into CLIP and generate the referential query to provide the prior context for decoder, along with a task-specific decoder. By incorporating the referential query into the decoder, we can effectively mitigate the learning difficulty of the decoder, and accurately concentrate on the target object. Additionally, our proposed query adaption module can also act as an adapter, preserving the rich knowledge within CLIP without the need to tune the parameters of the backbone network. Extensive experiments demonstrate the effectiveness and efficiency of our proposed method, outperforming state-of-the-art approaches on five visual grounding benchmarks.

==> table/ablation_backbone.tex <==

\begin{table}[tb!]
\setlength{\abovecaptionskip}{1.0mm} 
\caption{Ablation study of the RefFormer position on RefCOCOg.}
\label{tab:ablation_many}
\centering
\scalebox{1.0}{
\begin{tabular}{lcccccccc}
\toprule
Method &val &test \\ 
\hline
\textit{Backbone:}\\
Swin+Bert &75.25 & 75.61\\
\hline
\textit{Auxiliary loss:}\\
W/o $\mathcal{L}_{aux}$ &74.24	&73.82\\
\hline
\textit{Learnable queries:} \\
Referential query &52.92 &51.87\\
Linguistic embeddings &71.36 &71.07 \\
Random initialization
&73.40 &73.12 \\
\hline
Ours &75.84  &75.32 \\
\bottomrule
\end{tabular}
}
\end{table}

==> table/ablation_decoder.tex <==












\begin{table}[tb!]
\setlength{\abovecaptionskip}{1.0mm} 
\caption{Ablation study of learnable queries. }
\label{tab:ablation_decoder}
\centering
\scalebox{1.0}{
\begin{tabular}{l|cccccccc}
\toprule
Decoder layer &1 &2 &3 &4 \\ 
\hline
val \\
test \\
\bottomrule
\end{tabular}
}
\end{table}

==> table/ablation_fusion_layer.tex <==




\begin{table}[tbp!]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\vspace{0.1cm}
\makeatletter\def\@captype{table}\makeatother
\caption{Ablation study of multi-level fusion on RefCOCOg. }
\label{tab:ablation_multi-level}
\scalebox{0.82}{
    \begin{tabular}{l|cccccccc}
    \toprule
    Fusion layer ($\mathcal{K}$) &val &test \\ 
    \hline
    % \multicolumn{1}{c|}{None} \\
    \multicolumn{1}{c|}{{\{4\}}} &65.42 \textcolor{myred}{(-9.31)} &65.12 \textcolor{myred}{(-9.02)} \\
    \multicolumn{1}{c|}{{\{8\}}} &73.31 \textcolor{myred}{(-1.42)} &72.47 \textcolor{myred}{(-1.69)} \\
    \multicolumn{1}{c|}{{\{12\}}} &74.73 &74.16 \\
    \hline
    \multicolumn{1}{c|}{{\{4,8\}}} &72.71 \textcolor{myred}{(-2.02)} &73.03 \textcolor{myred}{(-1.13)}\\
    \multicolumn{1}{c|}{{\{4,12\}}} &75.33 \textcolor{mygreen}{(+0.60)} &74.51 \textcolor{mygreen}{(+0.35)} \\
    \multicolumn{1}{c|}{{\{8,12\}}} &75.61 \textcolor{mygreen}{(+0.88)} &74.82 \textcolor{mygreen}{(+0.66)} \\
    % \multicolumn{1}{c|}{{\{3,5,11\}}} &- &- \\
    \rowcolor{light-gray0} \multicolumn{1}{c|}{{\{4,8,12\}}} &\textbf{76.33 \textcolor{mygreen}{(+1.60)} }  &\textbf{75.33 \textcolor{mygreen}{(+1.17)}} \\
    \bottomrule
    \end{tabular}
}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\centering
\vspace{0.05cm}
\makeatletter\def\@captype{table}\makeatother\caption{Comparison of learnable parameters. The symbol (*) represents the model is closed-source, and the data is accessed from the original paper.}
\label{tab:ablation_param}
\scalebox{0.85}{
    \begin{tabular}{l|cccccccc}
    \toprule
    Method &Params(M)  \\ 
    \hline
    Transvg  &144.00\\
    RefTR   &144.73 \\
    \rowcolor{light-gray0} Ours &29.20 \\
    
    \bottomrule
    \end{tabular}
}
\end{minipage}
% \vspace{-7pt} % 确保两个 minipage 在垂直方向上对齐
\end{table}





==> table/ablation_param.tex <==











\begin{table}[tb!]
\setlength{\abovecaptionskip}{1.0mm} 
\caption{Comparison of learnable parameters. Among them, Dynamic MDETR and Transvg++ are closed-source, thus, the data is accessed from the original paper.}
\label{tab:ablation_param}
\centering
\scalebox{1.0}{
\begin{tabular}{l|cccccccc}
\toprule
Method &Total(M) &Decoder(M) \\ 
\hline
Transvg &144.00 & 8.39\\
RefTR \\
Dynamic MDETR &- &7.99 \\
Transvg++  &$> 116.14$ &-\\
\rowcolor{light-gray0} Ours &29.20 & \\
\bottomrule
\end{tabular}
}
\end{table}

==> table/ablation_refformer_layer.tex <==
\begin{table}[tb!]
\setlength{\abovecaptionskip}{1.0mm} 
\caption{Ablation study of the RefFormer position on RefCOCOg.}
\label{tab:ablation_positiion}
\centering
\scalebox{1.0}{
\begin{tabular}{l|cccccccc}
\toprule
RefFormer layer &val &test \\ 
\hline
\multicolumn{1}{c|}{None} &65.50 & 65.54 \\ 
 \multicolumn{1}{c|}{{\{4,8,12\}}} &74.08 \textcolor{mygreen}{(+8.58)} &73.82 \textcolor{mygreen}{(+8.28)} \\
\rowcolor{light-gray0} \multicolumn{1}{c|}{{\{4,6,8,10,12\}}} &\textbf{76.33 \textcolor{mygreen}{(+10.83)}}  &\textbf{75.33 \textcolor{mygreen}{(+9.79)}}  \\
\multicolumn{1}{c|}{{\{2,4,6,8,10,12\}}} &75.84 \textcolor{mygreen}{(+10.34)} &75.32 \textcolor{mygreen}{(+9.78)} \\
\bottomrule
\end{tabular}
}
\end{table}

==> table/ablation_training_strategy.tex <==










\begin{table}[tb!]
\setlength{\abovecaptionskip}{1.0mm} 
\label{tab:ablation-prior}
\centering
\scalebox{1.0}{
\begin{tabular}{l|cccccccc}
\toprule
Learnable Queries &val &test \\ 
\hline
None &- &- \\
Finetune &- &- \\
\rowcolor{light-gray0} Ours &\textbf{76.33 \textcolor{mygreen}{(+2.93)}} &\textbf{75.33 \textcolor{mygreen}{(+3.21)}} \\
\bottomrule
\end{tabular}
}
\caption{Ablation study of learnable queries. }
\end{table}

==> table/seg_sota.tex <==


\begin{table*}[tb!]
\setlength{\abovecaptionskip}{2.0mm} 
\centering
\scalebox{0.5}{
\begin{tabular}{l|ccc|ccc|cc}
\toprule
{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{3}{c|}{\textbf{RefCOCO}}                                             & \multicolumn{3}{c|}{\textbf{RefCOCO+}}                                            & \multicolumn{2}{c}{\textbf{RefCOCOg}}                 \\
{}                                                                                                             & val                       & testA                     & testB                     & val                       & testA                     & testB                     & {val}   & test                      \\ \hline
MAttNet \textcolor{gray}{\tiny{CVPR2018}} \cite{luo2020multi}   &56.51 &62.37 &51.70 &46.67 &52.39 &40.08 &47.64 &48.61\\
MCN \textcolor{gray}{\tiny{CVPR2020}} \cite{luo2020multi}   &62.44 &64.20 &59.71 &50.62 &54.99 &44.69 &49.22 &49.40\\
LTS \textcolor{gray}{\tiny{CVPR2021}} \cite{jing2021locate} &65.43 &67.76 &63.08 &54.21 &58.32 &48.02 &54.40 &54.25\\
VLT \textcolor{gray}{\tiny{ICCV2021}} \cite{}  &65.65 &68.29 &62.73 &55.50 &59.20 &49.36 &52.99 &56.65\\
RefTR \textcolor{gray}{\tiny{NIPS2021}}  \cite{li2021referring} &70.56 &73.49 &66.57 &61.08 &64.59 &52.73 &58.73 &58.51 \\
SeqTR \textcolor{gray}{\tiny{ECCV2022}} \cite{zhu2022seqtr} &67.26 &69.79 &64.12 &54.14 &58.93 &48.19 &55.67 &55.64\\
VG-LAW \textcolor{gray}{\tiny{CVPR2023}}  \cite{su2023language} & 75.05  & 77.36 & 71.69 & 66.61  & 70.30 & 58.14 & 65.36  & 65.13                    \\
PVD \textcolor{gray}{\tiny{AAAI2024}} \cite{cheng2024parallel}&74.82 &77.11 &69.52 &63.38 &68.60 &56.92 &63.13 &63.62\\
\hline 
Ours  &74.47 &\textbf{77.92} &\textbf{72.30} &\textbf{66.70} &\textbf{72.28} &\textbf{60.43} &\textbf{65.51} &\textbf{66.26} \\
\bottomrule
\end{tabular}
}
\caption{Comparisons with the state-of-the-art dense grounding approaches on three benchmarks for RES task, i.e., RefCOCO \cite{yu2016modeling}, RefCOCO+  \cite{yu2016modeling}, RefCOCOg~\cite{mao2016generation}. 
}
\label{tab:sota_refcoco_seg}
\end{table*}




